Prompting Contrastive Explanations for Commonsense Reasoning Tasks

Many commonsense reasoning NLP tasks involve choosing between one or more possible answers to a question or prompt based on knowledge that is often implicit. Large pretrained language models (PLMs) can achieve near-human performance on such tasks, while providing little human-interpretable evidence of the underlying reasoning they use. In this work, we show how to use these same models to generate such evidence: inspired by the contrastive nature of human explanations, we use PLMs to complete explanation prompts which contrast alternatives according to the key attribute(s) required to justify the correct answer (for example, peanuts are usually salty while raisins are sweet). Conditioning model decisions on these explanations improves performance on two commonsense reasoning benchmarks, as compared to previous non-contrastive alternatives. These explanations are also judged by humans to be more relevant for solving the task, and facilitate a novel method to evaluate explanation faithfulfness.

==> archived/abstract.tex <==
  % Need for generative explanations and need to narrow down the possible space of such explanations
%   Commonsense reasoning tasks are designed to evaluate humans' commonsense and background knowledge that is generally underspecified in the input text.  
%   As pretrained language models (PLMs) achieve remarkable performance on these tasks, this knowledge may be embedded in the parameters of the model. In this work, we aim to elicit this knowledge as a human-readable natural language explanation.
%   % How to 
%   A key observation that helps constrain the possible space of free-form explanations is that plausible alternatives that solve the commonsense reasoning instance can be contrasted along discerning attributes that explain why one choice is more likely. Contrasting these alternatives is also a human-centered format for explaining model decisions.
% %   Example: A good one from Winogrand.
%   We show that prompting PLMs to complete contrastive language prompts and conditioning model decisions on the resultant 
% %   intermediate
%   textual excerpts i) improves performance in the zero-shot and fine-tuned setting on two commonsense tasks, ii) provides a novel way to manipulate explanation and quantify faithfulness of the model to the generated explanation and, iii) is judged to be more relevant to prediction by humans when compared to prior work in generative explanations.

  Many commonsense reasoning tasks like the Winograd Schema Challenge 
  require the comparison of two or more plausible alternatives in the input, one of which is more likely based on commonsense knowledge that is underspecified in the text. 
  Humans solve such tasks by \emph{contrasting} these alternatives along a discerning attribute such as size, density, etc.
  As pretrained language models (PLMs) achieve remarkable performance on these tasks, this contrastive knowledge may be embedded in the parameters of the model. 
  In this work, we aim to elicit this knowledge as a human-readable textual excerpt.
  We show that PLMs can be used to complete contrastive language prompts to generate contrastive explanations. 
  By conditioning model decisions on the these explanations, we improve task performance on two commonsense tasks. The completed prompts can be manipulated to quantify faithfulness of the model to the generated explanation. Finally, contrastive explanations are judged to be more relevant to prediction by humans when compared to prior work in explanation generation.
  
  % Luke's version
  Many NLP tasks involve choosing between one or more plausible textual answers to a question or prompt. Recent large language models can achieve near-human performance on many such tasks, while providing little human-interpretable evidence of the underlying reasoning they use. In this paper, we show it is possible to also use the same models to generate contrastive natural language explanations that compare the alternatives according to the key attribute(s) required to justify the correct answer (e.g. a child might prefer cake to brocolli because it is sweeter). Using a simple set of templates to prompt the model to consider such explicit comparisons, we show strong performance on two commonsense reasoning benchmarks, including a new state of the art for the zero-shot setting. This mechanism provides a new way to manipulate explanation to quantify faithfulness of the model, which we also show leads to explanations that are judged to be more faithful in human evaluations than previous non-contrastive alternatives.
  
  
    % Combined version after discussion with Luke
  Many commonsense reasoning NLP tasks involve choosing between one or more plausible answers to a question or prompt based on knowledge that is often implicit.
  Large pretrained language models (PLMs) can achieve near-human performance on such tasks, while providing little human-interpretable evidence of the underlying reasoning they use. 
  In this work, we are inspired by how humans typically solve such tasks -- by \emph{contrasting} the alternatives along a differentiating attribute (e.g. they may prefer peanuts over raisins as a savoury snack as peanuts are saltier).
  We use a simple set of templates to prompt the model to generate contrastive explanations that compare the alternatives according to the key attribute(s) required to justify the correct answer, thereby eliciting contrastive knowledge they may already contain.
  By conditioning model decisions on the these explanations, we improve performance on two commonsense reasoning benchmarks, including a new state of the art for the zero-shot setting. This mechanism also provides a new way to manipulate the explanation to quantify the model's faithfulness to it. Contrastive explanations are also judged more relevant for prediction by humans than previous non-contrastive alternatives.

==> archived/introduction_v1.tex <==

% \begin{figure}
% \centering
% \includegraphics[scale=0.30]{sections/resources/contrastive_winograd_example.pdf}
% \caption{Winograd Schema Instance:``I picked up a bag of peanuts and raisins for a snack. 
% I wanted a sweeter snack out so I stored the $\_$ for now." can be explained by contrasting the two choices - peanuts/raisins - on the basis of a specific characteristic like taste. \textit{Peanuts are salty while raisins are sweet.} is an instance of a contrastive explanation}
% \label{fig:contrastive_example}
% \end{figure}



% \textbf{Para1 : Why generate an explanation for CS tasks, and what's the challenge there}
% Explanation for some tasks needs to be generative. PLMs nearly solve this task. Space of possible human-readable explanations are infinite if generation is the way forward and this needs to be made tractable. Line of work where guided generation through the means of using prompts can help extract this knowledge from PLMs\\
As large pretrained language models (PLMs) continue to achieve staggering performance gains on standard NLP tasks, recent work has attempted to set more challenging goals for these models -- tasks that require commonsense reasoning that humans can solve with relative ease. This is because commonsense reasoning is implicit and underspecified in text.
% making this task challenging. 
For instance, determining filling in the Winograd schema instance \textit{``I picked up a bag of peanuts and raisins for a snack. I wanted a sweeter snack out so I ate the $\_$ for now."} with either peanuts or raisins requires information about these entities that is not specified in the input -- the distinguishing attribute of taste. Raisins are more likely to be sweeter than peanuts.
% , is an essential piece of reasoning missing from the text.
Surprisingly, PLMs achieve near-human performance on these benchmark tasks as well, while providing little human-interpretable evidence of the underlying reasoning used. 
This implicit reasoning maybe contained in the millions of parameters of the model, learned from massive textual data it was pre-trained on. Recent work on interpretability attempts to generate this reasoning as an intermediate natural language explanation \citet{latcinnik2020explaining, shwartz2020unsupervised}.
However, the space of all possible free-form explanations is exponentially large, making this generative process challenging. In this work we use contrastive prompts to constrain generation, improving on both, task performance and human evaluation.
% , we constrain this generative process using contrastive language prompts. Our contrastive explanations are grounded in a human-centered approach to explanation, improves task performance and are amenable to diagnosing model behavior.
% and we need to be able to find optimal ways of constraining this generative process. 


\begin{table}[]
    \centering
    \begin{tabular}{l}
    \toprule
        i) I picked up a bag of \textcolor{red}{peanuts} and \textcolor{green}{raisins} for \\ a snack. I wanted a sweeter snack out so I\\
         ate the $\_$ for now. \\ 
        \textit{Human: Peanuts are salty while raisins tend}\\ \textit{to be sweet.}\\
         \midrule
        ii) The geese prefer to nest in the \textcolor{green}{fields} rather \\ 
         than the \textcolor{red}{forests} because in the $\_$ predators \\
        are more hidden. \\
        \textit{Human: Forests are denser than fields}\\
    \bottomrule
    \end{tabular}
    \caption{Examples of Winograd Scheme Instances where the correct and incorrect answer choice are highlighted in green and red respectively. Choices are \emph{contrasted} along attributes like taste (for i) and density of vegetation (for ii) by humans to explain why they prefer some answer choice.} 
    \label{tab:_figure}
\end{table}


% \textbf{Para2: Why contrastive? Social (human-centered) inspiration}
% humans use contrast. As miller points our, people do not ask why event P happened, but rather why event P happened instead of some event Q, where Q is the foil. What kind of form does this take? Here is an example.
\citet{miller2018contrastive} systematically surveyed over 250 papers in philosophy, psychology, and cognitive science on how people explain to each other, and observed that explanations are contrastive. People do not ask``Why P?"; they ask ``Why P rather than Q?", where Q can be implicit from the context. For example, instead of justifying why peanuts is correct, humans explain why peanuts is more likely than raisins.  
A contrastive explanation 
% Here we need to define contrastive explanation.
% \textbf{Para2: Why contrastive? Computational tractability based inspiration}
\citet{miller2018contrastive} also argue that a contrastive explanation has additional computational benefits in that it limits the space of possible explanations. Instead of exhaustively enlisting all possible reasons an answer choice is correct, we only need to enlist the limited set of reasons that make one answer more likely than the other. For instance, the differentiating characteristic of taste between a peanut and a raisin is adequate to explain the example above. The peanut's size, temperature, color, etc are irrelevant attributes. 
% \citet{miller2018contrastive} also argues that 

% \textbf{What we do?}
 Motivated by the social and computational significance of contrastive explanations, we constrain PLMs to generate explanations that contrast plausible alternatives in the instance based on their distinguishing attributes. 
%  as intermediate reasoning while solving commonsense tasks. 
%  We introduce a generative explanation format that closely follows the way humans explain their decisions in the face of choice, by contrasting the choices based on their distinguishing attributes. 
 We develop a small set of contrastive language templates that can be in-filled by pretrained language models to generate contrastive text excerpts, which can then be combined with the original input. The models' final task prediction is conditioned on the original input and the generated contrastive excerpts. The contrastive templates we employ (see \ref{tab:contrastive_patterns}) are also amenable to diagnosing model dependence on the explanation when the generated contrast is reversed during evaluation - \emph{peanuts are sweet and raisins are salty}.
%  Our templates are also designed to be amenable to manipulation
 
% \textbf{What we observe}
% Perf. improves over baseline and previous attempts at extracting intermediate reasoning from PLMs. Contrastive evaluation (flipping the generated explanation) and Abstractive Evaluation provide insights on rationale faithfulness and input dependency. Humans deem our contrastive explanations to be much superior than self-talk patterns and unconstrained generation models. 
Our model  shows quantitative improvements in task performance over previous work \citet{shwartz2020unsupervised, latcinnik2020explaining} that has attempted to generate intermediate explanation for
% commonsense reasoning tasks. Our model achieves significant improvements in task performance over these methods for the same model size over 
two commonsense reasoning tasks - Winograd Schema Challenge \citet{kocijan2020review} and multiple-choice question answering about physical commonsense \citet{sap2019socialiqa}. Our gains in the zero-shot setting are especially notable, achieving SOTA with the largest open-source pretrained model and improving over \citet{shwartz2020unsupervised} by X\%. Improved task performance indicate better quality of intermediate explanation, which is further corroborated by our human evaluation study. Contrastive explanations are deemed more useful by humans than  prior techniques, especially in terms of relevance to the task and usefulness in making the decision.
Furthermore, reversing the generated contrastive explanation during evaluation hurts task performance by X\%, 
indicating the degree to which the model relies on the generated explanation as opposed to latent information in its parameters.
% while (b) Abstractive evaluation exposes the extent to which the model relies on the explanation if parts of the input are obscured.

% Contributions of the work include: 
% \begin{itemize}
%     \item We introduce a generative explanation format that closely follows the way humans explain their decisions in the face of choice, by contrasting the choices based on their distinguishing attributes.
%     \item We develop a small set of contrastive templates that can be in-filled by pretrained language models to generate these contrastive explanations , which are then used to make the task prediction. Our models can be further fine-tuned on the task.
%     \item We obtain significant improvements in task performance over baselines of the same model size for two commonsense tasks. Our gains in the zero-shot setting are especially notable, achieving SOTA with the largest open-source pretrained model. And.
%     \item Our human evaluation study indicates that contrastive explanations are deemed more useful by humans than prior techniques for free-form explanation generation
%     \item Our novel contrastive format allows for two additional tests of the generated explanations for faithfulness i.e. reliance of the model on the explanation (a) Contrastive evaluation indicates the degree to which reversed explanations can hurt model performance, while (b) Abstractive evaluation exposes the extent to which the model relies on the explanation if parts of the input are obscured. 
% \end{itemize}

% \textbf{More Observations} Contribution is a form of querying and extracting knowledge from models through prompts and templates, not a model itself. Contributions are orthogonal to the PLM being used.

==> archived/method_model.tex <==

%In order to operationalize the contrastive explanation theory in a straightforward manner,  we focus on reasoning tasks where the fact P and the foil Q are explicitly stated but the contrastive explanation itself is implicit. For instance, in the Winograd Schema challenge, P and Q are the two noun phrases that can be antecedents of an ambiguous pronoun in a statement and one of them is more likely than the other.  As demonstrated by the examples in Table \ref{tab:examples_contrastive}, this choice can be explained by differentiating these noun phrases along a specific attribute or property.


% All of this needs to shift to the part where we describe the model.
% We use these custom contrastive language prompts to generate explanations from the model. We are basically guiding the model's reasoning ability to be more akin to humans by asking it to complete these prompts and then conditioning its decision on what it has generated. Note that OPT1 and OPT2 stand, interchangeably, for the fact and foil.
% important replacement phrases: extracting contrastive knowledge instead of reasoning
% LMs dont do any internal contrasting -- the LM is just there to generate some phrases that look nice and plausible. The contrastive templates themselves force contrastive style statements, and combined with the classifier loss we hope it encourages contrasting to happen; though what "contrasting happening" means maybe isn't obvious...

% \subsection{Constructing Custom Prompts}
% \begin{itemize}
%     \item preprocessing to partially complete the template using NP and VP extraction - extracting the minimal difference to fill in the model.
%     \item filtering of more likely formats based on the type of NP/VP, task and surrounding context.
% \end{itemize}


% IDeal comparison should be how much can we recover back going from 3 to 4. It benefits those examples where the model has to rely on the entities itself. However what does that indicate? 


% THis should also include a discussion on how this relates to a counterfactual.
% Another argument : It measures how much the model uses explanation vs the common sense knowledge in the parameters of the model.

% \paragraph{Abstract Evaluation} 
% To further necessitate the use of the explanation, we use a setting where once the explanation is generated, we obscure the identity of the two alternatives to be contrasted while retaining their identities in the explanation itself. For example, the following input sequence is used while predicting the label -- ``I picked up a bag of OPT1 and OPT2 for a snack. I wanted a sweeter snack out so I ate the $\_$ for now. Peanuts are salty while raisins are sweet." A reduction in the model's performance is expected since the entities are obscured in the original input and the magnitude of this decline approximates the extent to which the model relies on the explanation. The smaller the decline, the more reliant the model is on the explanation.

% 1. ``I picked up a bag of peanuts and raisins for a snack. I wanted a sweeter snack out so I ate the $\_$ for now. Peanuts are salty while raisins are sweet." - best 
% 2. ``I picked up a bag of peanuts and raisins for a snack. I wanted a sweeter snack out so I ate the $\_$ for now." - better
% 3. ``I picked up a bag of OPT1 and OPT2 for a snack. I wanted a sweeter snack out so I ate the $\_$ for now. Peanuts are salty while raisins are sweet." - slightly worse.
% 4. ``I picked up a bag of OPT1 and OPT2 for a snack. I wanted a sweeter snack out so I ate the $\_$ for now. OPT1 are salty while OPT2 are sweet." - equally worse 
% 5. ``I picked up a bag of OPT1 and OPT2 for a snack. I wanted a sweeter snack out so I ate the $\_$ for now. " - equally worse 



